Fault Localization with Code Coverage Representation Learning

In this paper, we propose DeepRL4FL, a deep learning fault localization (FL) approach that locates the buggy code at the statement and method levels by treating FL as an image pattern recognition problem. DeepRL4FL does so via novel code coverage representation learning (RL) and data dependencies RL for program statements. Those two types of RL on the dynamic information in a code coverage matrix are also combined with the code representation learning on the static information of the usual suspicious source code. This combination is inspired by crime scene investigation in which investigators analyze the crime scene (failed test cases and statements) and related persons (statements with dependencies), and at the same time, examine the usual suspects who have committed a similar crime in the past (similar buggy code in the training data). For the code coverage information, DeepRL4FL first orders the test cases and marks error-exhibiting code statements, expecting that a model can recognize the patterns discriminating between faulty and non-faulty statements/methods. For dependencies among statements, the suspiciousness of a statement is seen taking into account the data dependencies to other statements in execution and data flows, in addition to the statement by itself. Finally, the vector representations for code coverage matrix, data dependencies among statements, and source code are combined and used as the input of a classifier built from a Convolution Neural Network to detect buggy statements/methods. Our empirical evaluation shows that DeepRL4FL improves the top-1 results over the state-of-the-art statement-level FL baselines from 173.1% to 491.7%. It also improves the top-1 results over the existing method-level FL baselines from 15.0% to 206.3%.

==> sections/motiv_overview.tex <==
\subsection{Overview of Our Approach}



Figure~\ref{overview} shows {\tool}'s overview with three key
representation learning processes: code coverage representation
learning (dynamic information), statements dependency representation
learning (both dynamic and static information), and source code representation learning
(static information).

{\bf For code coverage representation learning,} we first collect the
details of a code coverage matrix from given test cases
(Figure~\ref{fig:motiv_example1_b}).  We then perform the analysis on
the output of tests cases to locate the error-exhibiting (EE) lines
of code. Basically, if the execution of a test crashes, the line
information is always available. Even if the test fails, the program
often explicitly lists the lines of code that exhibit the
incorrect results/behaviors. We use such information to locate EE lines
in the buggy source code (Section~\ref{1.1}). 
The row in the code
coverage matrix corresponding to the EE lines will be marked with all
-1 values. After that, we perform a reordering on the columns of the
code coverage (CC) matrix by evaluating the lines of code that each
test case runs through. The goal is to form ``visual'' characteristic
feature in the matrix by grouping the test cases that run through
similar lines of code. The resulting matrix at this step is called
enhanced CC matrix (ECC matrix). We expect a deep learning model such
as CNN can recognize those visual characteristics to detect the buggy
method and lines of code. The ECC matrix will be the input for our
spectrum-based/mutation-based representation learning process in which
the information in the ECC matrix is encoded into the representation
vectors for the CNN model.


{\bf For statement dependency representation learning,} we consider
both dynamic and static information. For the dynamic part, we consider
the statements in the execution order in the test cases. However, if
the statements are executed sequentially in the same nested level as
part of a block statement, they would give the same suspiciousness
score by the spectrum-based approaches (see motivating
examples). Therefore, to address the issue, we consider also the data
dependencies among the statements nested within a block
statement. Specifically, we collect execution paths and data flow
graph for each test case. We use word2vec~\cite{word2vec} and
node2vec~\cite{Grover-2016} to generate the representation vectors
with these paths and graphs for the encoding of them.

{\bf For source code representation learning,} we first build the AST
from the source code. From the AST, we choose to represent the code
structure by the long paths that are adapted from a prior
work~\cite{Alon-2018,yioopsla19}. A long path is a path that starts
from a leaf node and ends at another leaf node and passes the root
node of the AST. The AST structure can be captured and represented via
the paths with certain lengths across the AST
nodes~\cite{Alon-2018}. The reason for a path to start and end at leaf
nodes is that the leaf nodes in an AST are terminal nodes with
concrete lexemes. The nodes in a path are encoded into a continuous
vector.  We also integrate into our representation the token
representation and statement representation (Section~\ref{4}). The
output of this code representation learning is the vector
representing the buggy code, which will be used as input of the CNN
model for fault localization.


%\begin{itemize}
	
%	\item \textbf{Test Coverage Representation Learning}.  First,
%          our model parses all test cases and collect the code
%          coverage information that shows which statement covered by
%          which test cases. And then, we also collect the error
%          position for the failed test cases. With these two kind of
%          information, we generate improved code coverage
%          matrix. After generation, we re-ordered test cases in the
%          matrix based on the number of failure and covered test
%          cases. With these steps, we call it spectrum-based way. We
%          also do this work on mutation-based way. The mutation-based
%          way means that for each mutater, we replace changed
%          statement into the original method and collect improved code
%          coverage matrix for them.
	
%	\item \textbf{Code Representation Learning}.
%	Second, in order to considering the given statement source code, we use code representation tool to represent each statement in order to catch the tokens relationship in each statement. With the tool, we can generate statement representation vectors in this step.
	
%	Also, we consider the relationship among statements. we collect execution paths and data flow graph [] for each test case. We use word2vec [] and node2vec [] to generate the representation vectors with these paths and graphs for the encoding of them.

Finally, all representation vectors including spectrum based
representation vectors, mutation-based representation vectors, 
statement dependency representation vectors, and source code vectors 
are used as the inputs of a
CNN model that acts as the classifier for each statement or 
method as buggy or not.
%We use CNN to analyze the relations inside of the code coverage
%matrix, and between the source code and its code coverage matrix.
For classification, we use a softmax-based CNN classifier.

%	\textbf{Fault Localization}.  Third, we combine the improved
%        code coverage matrix we got in step 1 with the encoding
%        vectors from execution path and data flow graph in step 2
%        together. With this bigger matrix, we use CNN [] model to
%        extract relationship information inside of these matrix with
%        representation vectors for both spectrum and mutation based
%        ways.
	
%	In the end, we collect spectrum based representation vectors,
%        mutation based representation vectors and statement
%        representation vectors to locate the faults by using a CNN []
%        model to classify each statement in the given project.

%        In the step of Fault Localization, we all use CNN [] model to
%        deal with the matrix and to the classification. Because the
%        CNN has been proved that it can work well in extracting useful
%        information inside of matrix, we use CNN to analysis the
%        relationship information inside of the matrix. And for
%        classification, with the representation vectors we can do the
%        fault localization with a softmax-based CNN classifier. CNN
%        has been proved can often works well on classification
%        problems in many existing studies []. We will explain all the
%        steps in details next.

        
%\end{itemize}







%In the step of Test Coverage Representation Learning, we use the code coverage tool [] to do the analysis. This tool can also provide the error position information for each failed test case. With the tool of this, we can generate the improved code coverage matrix which is the matrix that has the rows represent statements, has the columns represent test cases, and filled by 1, 0, and -1 to represent covered, not covered, and covered but failed. What's more, for the mutation based ways, we use the existing framework [] to try possible mutators and get improved code matrix from them. We use both spectrum based way and mutation based way is that we would like to extract as much relationship among test cases, code coverage, and possible fixes as I can in order to improve the fault localization.

%In the step of Code Representation Learning, we use well known tool word2vec [] on the representation learning area to get the token representation vectors. The word2vec can help us collect the token relationship inside of each statement and get the representation vector for each statement. Also, in this step, we use execution paths and data flow graph [] to represent the relationship among statements. Using execution paths is because it can show the real control dependency happens for each test case which can reduce the biases when comparing with others, such as control flow graph. We use data flow graph is because when we want to analysis the code inside of a code block such as for loop, the execution path will go through the code again and again which will reduce the relationship between the code inside of the code block and the code outside of the code block. The data flow graph can help us solve this problem. Because the data flow graph only consider the data changes, even in the code block, it still will be linked to the code outside of the code block which can show the data dependency well. That's why we use them in this step.

%In the step of Fault Localization, we all use CNN [] model to deal with the matrix and to the classification. Because the CNN has been proved that it can work well in extracting useful information inside of matrix, we use CNN to analysis the relationship information inside of the matrix. And for classification, with the representtion vectors we can do the fault localization with a softmax-based CNN classifier. CNN has been proved can often works well on classification problems in many existing studies []. We will explain all the steps in details next.




